Topological defects in string theory orbifolds with target spaces $\mathbb{C}/\mathbb{Z}_N$ and $S^1/\mathbb{Z}_2$

We study conformal defects in two important examples of string theory orbifolds. First, we show that topological defects in the language of Landau-Ginzburg models carry information about the RG flow between the non-compact orbifolds $\mathbb{C}/\mathbb{Z}_d$. Such defects are shown to correctly implement the bulk-induced RG flow on the boundary. Secondly, we study what the possible conformal defects are between the $c=1$ bosonic 2D conformal field theories with target space $S^1/\mathbb{Z}_2$. The defects cataloged here are obtained from boundary states corresponding to D-branes in the $c=2$ free theory with target space $S^1/\mathbb{Z}_2 \times S^1/\mathbb{Z}_2$. Via the unfolding procedure, such boundary states are later mapped to defects between the circle orbifolds. Furthermore, we compute the algebra of the topological class of defects at different radii.

==> data/appendices.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  New template code for TAMU Theses and Dissertations starting Fall 2016.  
%
%
%  Author: Sean Zachary Roberson 
%	 Version 3.17.01
%  Last updated 1/10/2017
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{appendices}
\titleformat{\chapter}{\centering\normalsize}{APPENDIX \thechapter}{0em}{\vskip .5\baselineskip\centering}
\renewcommand{\appendixname}{APPENDIX}

\input{data/appendix1}
\input{data/appendix2}

\end{appendices}

==> data/bibliography.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  New template code for TAMU Theses and Dissertations starting Fall 2016.
%
%  Author: Sean Zachary Roberson
%	 Version 3.16.09
%  Last updated 9/12/2016
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                           REFERENCES 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\phantomsection
\addcontentsline{toc}{chapter}{REFERENCES}

\renewcommand{\bibname}{{\normalsize\rm REFERENCES}}

%\bibliographystyle{ieeetr}
\bibliography{data/myReference}

==> data/contributors.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  New template code for TAMU Theses and Dissertations starting Fall 2016.  
%
%
%  Author: Sean Zachary Roberson
%	 Version 3.17.01 
%  Last updated 1/10/2017
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%             CONTRIBUTORS AND FUNDING SOURCES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\chapter*{CONTRIBUTORS AND FUNDING SOURCES}
\addcontentsline{toc}{chapter}{CONTRIBUTORS AND FUNDING SOURCES}  % Needs to be set to part, so the TOC doesn't add 'CHAPTER ' prefix in the TOC.


%This section is taken directly from the MS Word templates.

%Old version below.

%All theses and dissertations must include a contributors and funding sources section. In this section, name all members of the dissertation committee, and any collaboration with others in carrying out your thesis or dissertation research. Your independent contributions must be made clear.
%
%If financial support from the university or any other source was gained to conduct your thesis or dissertation research and compilation, it must be listed in this section. If you completed all work independently without outside financial support, indicate this here.
%\textit{(Sample Wording)}
%
%This work was supported by a dissertation committee consisting of Professor XXX [advisor – also note if co-advisor] and XXXX of the Department of [Home Department] and Professor(s) XXXX of the Department of [Outside Department].
% 
%The data analyzed for Chapter III was provided by Professor XXXX. The analyses depicted in Chapter IV were conducted in part by Rebecca Jones of the Department of Biostatistics and were published in (year) in an article listed in the Biographical Sketch. 
%
%All other work conducted for the dissertation was completed by the student independently.
%
%\noindent \textit{(or)}
%
%This work was supervised by a dissertation committee consisting of Professor XXXX [advisor – also note if co-advisor] and Professor(s) XXXX of the Department of [Home Department] and Professor(s) XXXX of [Outside Department]. All work for the dissertation was completed independently by the student.
%
%\noindent \textit{(or)}
%
%Graduate study was supported by a fellowship from Texas A\&M University and a dissertation research fellowship from XXX Foundation.

\subsection*{Contributors}
This work was supported by a thesis (or) dissertation committee consisting of Professor XXXX [advisor --– also note if co-advisor] and XXX of the Department of [Home Department] and Professor(s) XXXX of the Department of [Outside Department].

The data analyzed for Chapter X was provided by Professor XXXX. The analyses depicted in Chapter X were conducted in part by Rebecca Jones of the Department of Biostatistics and were published in (year) in an article listed in the Biographical Sketch.

All other work conducted for the thesis (or) dissertation was completed by the student independently.
\subsection*{Funding Sources}
Graduate study was supported by a fellowship from Texas A\&M University and a dissertation research fellowship from XXX Foundation. 
\pagebreak{}

==> data/nomenclature.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  New template code for TAMU Theses and Dissertations starting Fall 2016.
%
%
%  Author: Sean Zachary Roberson
%	 Version 3.17.01
%  Last updated 1/10/2017
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                           NOMENCLATURE
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\chapter*{NOMENCLATURE}
\addcontentsline{toc}{chapter}{NOMENCLATURE}  % Needs to be set to part, so the TOC doesnt add 'CHAPTER ' prefix in the TOC.

%A note about aligning: These entries will align
%themselves according to the ampersand (&).
%No extra spaces are needed, as seen in some of
%the entries below.

%Example of the longtable environment.
\vspace{18pt}
\begin{spacing}{1.0}
	\begin{longtable}[htbp]{@{}p{0.33\textwidth} p{0.62\textwidth}@{}}
	   % \begin{tabular}{@{}p{0.33\textwidth} p{0.62\textwidth}@{}}
		OGAPS	&	Office of Graduate and Professional Studies at Texas A\&M University\\	[2ex]
		B/CS		&	Bryan and College Station\\	[2ex] %[2ex] provides double space between each row
		TAMU			&	Texas A\&M University\\	[2ex]
		SDCC & San Diego Comic-Con\\ [2ex]
		EVIL & Every Villain is Lemons\\ [2ex]
		EPCC & Educator Preparation and Certification Center at Texas A\&M University - San Antonio\\ [2ex]
		FFT & Fast Fourier Transform\\ [2ex]
		ARIMA & Autoregressive Integrated Moving Average\\ [2ex]
		SSD & Solid State Drive\\ [2ex]
		HDD & Hard Disk Drive\\ [2ex]
		O\&M & Eller Oceanography and Meteorology Building\\ [2ex]
		DOS & Disk Operating System\\ [2ex]
		HDMI & High Definition Multimedia Interface\\ [2ex]
		$L^1$ & Space of absolutely Lebesgue integrable functions; i.e., $\int |f| < \infty$\\ [2ex]
		$L^2$ & Space of square-Lebesgue-integrable functions, i.e., $\int |f|^2 < \infty$\\ [2ex]
		$PC(S)$ & Space of piecewise-continuous functions on $S$\\ [2ex]
		GNU & GNU is Not Unix\\ [2ex]
		GUI & Graphical User Interface\\ [2ex]
		PID & Principal Integral Domain\\ [2ex]
		MIP & Mixed Integer Program\\ [2ex]
		LP & Linear Program\\ [2ex]
		%XXXXXXXX		&	This is an optional page. Random word to test how long the sentence can be? This is just for test purpose. The current setting aims to align left/right margin same as all other pages.\\	[2ex]
	   % \end{tabular}%
	\end{longtable}
\end{spacing}

\pagebreak{}
